Houdini: Fooling Deep Structured Prediction Models

Generating adversarial examples is a critical step for evaluating and improving the robustness of learning machines. So far, most existing methods only work for classification and are not designed to alter the true performance measure of the problem at hand. We introduce a novel flexible approach named Houdini for generating adversarial examples specifically tailored for the final performance measure of the task considered, be it combinatorial and non-decomposable. We successfully apply Houdini to a range of applications such as speech recognition, pose estimation and semantic segmentation. In all cases, the attacks based on Houdini achieve higher success rate than those based on the traditional surrogates used to train the models while using a less perceptible adversarial perturbation.

==> 03-adv-examples.tex <==
\section{Adversarial Examples}
\label{adv-expm}
\subsection{Adversarial examples}
\label{sec:advex}
Given an input (train or test) example $(\bx, \by)$, an adversarial
example is a perturbed version of the original pattern $\adv{\bx} = \bx +
\perturb{\bx}$ where $\perturb{\bx}$ is small enough for 
$\adv{\bx}$ to be undistinguishable from $\bx$ by a human, but causes the network to predict an
incorrect label. Given the network parameters and structure $g(.,
\params)$ and a $p$-norm, the adversarial example is formally defined as
\begin{equation}
\label{eq:adv}
\bxprime = \argmax_{\bxprime:\normp{\bxprime-\bx}\leq \adveps}
\loss\big(\network(\bxprime, \params), \by\big)\,,
\end{equation}
where $\adveps$ represents the strength of the adversary. Since the
optimization problem above is non-convex,
\cite{shaham2015understanding} propose to take the first
order taylor expansion of $\bx\mapsto\loss(\network(\bx, \params),
\by)$ to compute $\perturb{\bx}$ by solving
\begin{equation}
\label{eq:fgsm}
\bxprime = \argmax_{\bxprime:\normp{\bxprime-\bx}\leq \adveps}
\big(\nabla_{\bx} \loss(\network(\bx, \params),
\by)\big)^T (\bxprime-\bx)\,.
\end{equation}
If $p=\infty$, then $\bxprime = \bx + \adveps \text{sign}(\nabla_{\bx}
\loss(\network(\bx, \params), \by))$. This is the \emph{fast gradient
  sign method}. For the case $p=2$, we obtain $\bxprime = \bx + \adveps
\nabla_{\bx} \loss(\network(\bx, \params), \by)$. A more involved
method is the \emph{iterative fast gradient sign method}, in which
several gradient steps of \eqref{eq:fgsm} are performed with a smaller
stepsize to obtain a local minimum of \eqref{eq:adv}.

